An Empirical Study of Low Precision Quantization for TinyML

Tiny machine learning (tinyML) has emerged during the past few years aiming to deploy machine learning models to embedded AI processors with highly constrained memory and computation capacity. Low precision quantization is an important model compression technique that can greatly reduce both memory consumption and computation cost of model inference. In this study, we focus on post-training quantization (PTQ) algorithms that quantize a model to low-bit (less than 8-bit) precision with only a small set of calibration data and benchmark them on different tinyML use cases. To achieve a fair comparison, we build a simulated quantization framework to investigate recent PTQ algorithms. Furthermore, we break down those algorithms into essential components and re-assembled a generic PTQ pipeline. With ablation study on different alternatives of components in the pipeline, we reveal key design choices when performing low precision quantization. We hope this work could provide useful data points and shed lights on the future research of low precision quantization.

==> abstract.tex <==
Tiny machine learning (tinyML) has emerged during the past few years aiming to deploy machine learning models to embedded AI processors with highly constrained memory and computation capacity. Ultra-low precision quantization is an important model compression technique that can greatly reduce both memory consumption (e.g., $\times 16$ reduction for 2bit quantization) and computation cost of a model. In this study, we focus on post-training quantization (PTQ) algorithms that quantize a model with only a small set of calibration data and benchmark them on different TinyML usecases. To achieve that under a fair setting, we build a simulated quantization framework to investigate recent PTQ algorithms. Furthermore, we deconstruct them into essential components and assemble a generic PTQ pipeline. With ablation study on different alternatives of components in the pipeline, we reveal key design choices when performing ultra-low precision quantization. We hope this work provide useful data points and shed lights on future research on ultra-low precision quantization.
